Multi-task Bias-Variance Trade-off Through Functional Constraints

Multi-task learning aims to acquire a set of functions, either regressors or classifiers, that perform well for diverse tasks. At its core, the idea behind multi-task learning is to exploit the intrinsic similarity across data sources to aid in the learning process for each individual domain. In this paper we draw intuition from the two extreme learning scenarios -- a single function for all tasks, and a task-specific function that ignores the other tasks dependencies -- to propose a bias-variance trade-off. To control the relationship between the variance (given by the number of i.i.d. samples), and the bias (coming from data from other task), we introduce a constrained learning formulation that enforces domain specific solutions to be close to a central function. This problem is solved in the dual domain, for which we propose a stochastic primal-dual algorithm. Experimental results for a multi-domain classification problem with real data show that the proposed procedure outperforms both the task specific, as well as the single classifiers.

==> latex_resources/my_sections.tex <==
\usepackage{needspace}

% \nbsubsection{} provides a numbered subsection in bold without a line break. The section will contain at least three lines of text before a pagebreak
\newcommand{\nbsubsection}[1]{\needspace{1\baselineskip}\color{white}\medskip\subsection{#1}\vspace{-3\baselineskip}\color{black}\medskip{\noindent \bf \thesubsection\quad #1.}}



% \nbsubsubsection{} provides a numbered subsection in bold without a line break. The section will contain at least three lines of text before a pagebreak
\newcommand{\nbsubsubsection}[1]{\needspace{1\baselineskip}\color{white}\subsubsection{#1}\vspace{-3\baselineskip}\color{black}\medskip{\noindent \bf \thesubsubsection. #1.}}

% \myparagraph provides a paragraph title in italics. 
\newcommand{\myparagraph}[1]{\needspace{1\baselineskip}\medskip\noindent {\it #1.}}

% \myindenetedparagraph provides an indented paragraph with title in italics.
\newcommand{\myindentedparagraph}[1]{\needspace{1\baselineskip}\medskip \hangindent=11pt \hangafter=0 \noindent{\it #1.}}

% \myparagraphtc provides a paragraph title in italics. It adds an enter to the table of contents
\newcommand{\myparagraphtc}[1]{\needspace{1\baselineskip}\medskip\noindent {\it #1.}\addcontentsline{toc}{subsubsection}{\qquad\qquad\quad#1}}



==> latex_resources/plot_appearance.tex <==


% This command sets the appearance of axis on pgfplots
\pgfplotsset{ ylabel near ticks,                 % Make x axis label appear close to figure
              xlabel near ticks,                 % Make y axis label appear close to figure
              tick label style = {font=\tiny},   % Write numbers in tiny font
              label style = {font=\tiny},        % Write axes labels in tiny size font
              title style = {font=\tiny},        % Write figure titles in tiny size font
            }

% style to draw dots in comb plots 
\tikzstyle{dot}          =[circle, draw=none, inner sep=0pt, minimum size =1.5mm, fill=black]
\tikzstyle{red dot}      =[dot, fill=red]
\tikzstyle{blue dot}     =[dot, fill=blue ]
\tikzstyle{red blue dot} =[dot, draw, thick, minimum size =1.2mm, red, fill=blue]
\def \greenfill {mygreen!40}

==> reply_reviewers.tex <==
Reviewer 2735	

This paper proposes a method for training GNNs that are stable to perturbations of their graph shift operator. I found the paper relatively easy to follow, even though I am not well versed in GNNs. I followed the derivation and thought the approach is well thought out. 

My only critique is that the experimental section is unclear in terms of how the dataset maps to the GNN. In other words, what are the nodes and edges? What is the optimization objective? For the non-expert reader, such as myself, the results section is key and it's important that the authors make this section clearer.

\red{We thank the reviewer for such a useful critique. We are glad to know that the reviewer found our paper of sufficient interest, and very original. 

In order to address the reviewers' concerns regarding the experimental section, let us clarify the section more in detail. First, to construct a graph, we use as nodes the movies, and the edges are the weight given by the graph similarity matrix obtained using the pairwise correlations between the different movies in the training set (an in depth explanation of this calculation can be found in [18]). In it's vanilla form, the objective is to minimize the L-1 loss, in our constrained version, the stability constraint is added. 

We only study the problem of predicting the rate a user would give to the movie 'Contact'. Therefore, given a user ratings, a graph signal is constructed, assigning each rating to each node (in this case movie). If a rating is not present, we assign a zero to it. The output of the GNN is likewise a graph signal, but we are only interested in the prediction of the movie 'Contact'. Therefore, the i-th output of the GNN (the one associated with 'Contact') is compared to the true value of the label, according to the L-1 loss.

We thank the reviewer for the useful comments, and we will add a better explanation of the numerical results to the body of the paper.}

# Reviewer 1717

- It seems to have a very limited work on the topics beside author's own research group which makes one wonder if the topic is of broad interest for the research community
- Most of the references are from author's own research group which makes it difficult to determine the significance of the contribution or even there is any interest on the topic beside author's own curiosity.

- It is hard to interpret what perturbation looks like in the context of movie similarity. An intuitive explanation on what perturbation might look like in this context would be very helpful. Or is this experiment purely theoretical simulation without any real world usefulness?
- Does the constrained learning need to know the 'magnitude of perturbation' for its training process? If it does then is the method practical for real world application especially when this 'magnitude of perturbation' is a theoretical parameter proposed by the authors.

\red{
We thank the reviewer for the useful review, we provide a detailed explanation of each of the elements that the reviewer alludes to. 

## References

We agree with the reviewer in that the references can be improved in order to motivate the importance of the problem under consideration. As the reviewer points out, stability of GNNs is a topic that has not been extensively studied, and therefore references are not plentiful.  However, stability and robustness of neural networks (in general not only graph), is an area of research that has received a great amount of attention lately. We will add the citations below, where the topic of Stability of GNNs is studied through the lens of robustness.

@misc{arghal2021robust,
      title={Robust Graph Neural Networks via Probabilistic Lipschitz Constraints}, 
      author={Raghu Arghal and Eric Lei and Shirin Saeedi Bidokhti},
      year={2021},
      eprint={2112.07575},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@inproceedings{jin2020graph,
  title={Graph structure learning for robust graph neural networks},
  author={Jin, Wei and Ma, Yao and Liu, Xiaorui and Tang, Xianfeng and Wang, Suhang and Tang, Jiliang},
  booktitle={Proceedings of the 26th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
  pages={66--74},
  year={2020}
}

@inproceedings{luo2021learning,
  title={Learning to drop: Robust graph neural network via topological denoising},
  author={Luo, Dongsheng and Cheng, Wei and Yu, Wenchao and Zong, Bo and Ni, Jingchao and Chen, Haifeng and Zhang, Xiang},
  booktitle={Proceedings of the 14th ACM International Conference on Web Search and Data Mining},
  pages={779--787},
  year={2021}
}

## Interpretation of Perturbation

In the case of the recommendation system considered in this paper, the perturbation is carried out over the movie similarity graph. The movie similarity graph is a symmetric matrix and is obtained computing the pairwise correlations between the different movies in the training set. Therefore, intuitively, adding a symmetric term, can be thought of as a perturbation of the training set, where the correlations between movies are modified according to the norm of $E$.

## Perturbation Magnitude

We thank the reviewer for allowing us to further explain this more in detail. It is not needed to know the magnitude of the perturbation $\epsilon$. It is the practitioner's job to determine the value of the constraint $C \epsilon$ that works the best in practice. In our case, we carried out an ablation study over $C \epsilon$ and presented the values of the best results. It must be noted that $\epsilon$ does not need to be known, for simplicity of exposition we chose to present the results as $C \epsilon$, but another constant i.e. $\gamma=C\epsilon$ could have been used (without knowledge of $\epsilon$. }



# Reviewer 0D05

In this work, the authors propose a constrained learning formulation to improve the stability of GNN. The experiment shows their proposed method can get benchmarked in the recommendation task. However, there are some suggestions. 1. the important result in the table can be shown in bold text. 2. A notation table would be very helpful since a lot of symbols are defined. 

\red{We thank the reviewer for the useful comments. We will take into account the reviewer's opinion, and we will add bold text in our results. We will try to add a table with notation, however, it may not be possible given the lack of available space.}
